CAMMARL: Conformal Action Modeling in Multi Agent Reinforcement Learning

Before taking actions in an environment with more than one intelligent agent, an autonomous agent may benefit from reasoning about the other agents and utilizing a notion of a guarantee or confidence about the behavior of the system. In this article, we propose a novel multi-agent reinforcement learning (MARL) algorithm CAMMARL, which involves modeling the actions of other agents in different situations in the form of confident sets, i.e., sets containing their true actions with a high probability. We then use these estimates to inform an agent's decision-making. For estimating such sets, we use the concept of conformal predictions, by means of which, we not only obtain an estimate of the most probable outcome but get to quantify the operable uncertainty as well. For instance, we can predict a set that provably covers the true predictions with high probabilities (e.g., 95%). Through several experiments in two fully cooperative multi-agent tasks, we show that CAMMARL elevates the capabilities of an autonomous agent in MARL by modeling conformal prediction sets over the behavior of other agents in the environment and utilizing such estimates to enhance its policy learning.

==> chapters/04_experiments.tex <==
In this section, we discuss the cooperative tasks with two agents used in this study (Figure~\ref{fig:envs}). We note here that though we work in fully cooperative settings in this article, \algo\ as an idea can be generalized to competitive or mixed settings too. 

\subsection{Environments}
We focus on two cooperative multi-agent environments illustrated in Figure~\ref{fig:env-cn} \&~\ref{fig:env-lbf}. Further details on these environments are in the supplementary material.

\begin{figure}[ht] 
\centering
\subfigure[]{
    \centering
    \includegraphics[width=0.5\linewidth]{images/cooperative_navigation.png} }
    % \caption{}
    % \caption{\textbf{Cooperative Navigation}: Agents (blue) learn to cover the two landmarks (black) avoiding collisions.} 
    \label{fig:env-cn}
% \end{subfigure}
\subfigure[]{
    \includegraphics[width=0.5\linewidth]{images/lbf.png}} 
    % \caption{}
    % \caption{} 
    \label{fig:env-lbf}
% \end{subfigure}
\caption{Multi-agent cooperative environments used in this study: (a) OpenAI MPE's \textbf{Cooperative Navigation}: Agents (blue) learn to cover the two landmarks (black) avoiding collisions. The figure shows \textbf{\acrlong{cn}} with 2 agents (N=2) and 2 landmarks (L=2). and (b) \textbf{Level-based foraging}: Agents must collect food and learn to cooperate using sparse rewards. This is a 12 $\times$ 12 \textbf{\acrlong{lbf}} grid-world with 2 cooperative players and 4 food locations.} 
\label{fig:envs}
\end{figure}

% \paragraph{Cooperative Navigation (\acrshort{cn})~\citep{mordatch2017emergence,lowe2017multi}.} In this task, agents are expected to learn to navigate and cover all the landmarks cooperatively and without colliding. 
% Each agent can perceive the other agents and landmarks within its reference frame (in the form of relative positions and velocities) and can take discrete actions to move around (left, right, up, down, stay) in the environment. The agents receive a team reward (so $r_{self}$ and $r_{other}$ are the same in this case) which is calculated as the minimum of the distance of the agents’ and landmarks’ ($x_i$, $y_i$) positions in the grid world. This reward, based on their proximity (or distance) from each of the landmarks, forces the need for cooperation in order to succeed in the task. Furthermore, agents are penalized upon collisions. Formally, the reward function in this environment can be defined as \[ r = \left[ -1 * \sum_{l=1}^{L} min_{\{n \in \mathcal{N}\}} ( distance(n, l) ) \right] - c \] where $|\mathcal{N}|$ is the number of agents and L are the landmarks in the environment. Here, c is the number of collisions in an episode and the agents are penalized with -1 for each time two agents collide. Figure~\ref{fig:env-cn} shows an illustration of this environment. 

% \paragraph{Level-based foraging (\acrshort{lbf})~\citep{albrecht2015game}.} In this environment, $\mathcal{N}_{self}$ and $\mathcal{N}_{other}$ are part of a 12$\times$12 grid world which contains four randomly scattered food locations, each assigned a level. The agents also have a level of their own. They attempt to collect food which is successful only if the sum of the levels of the agents involved in loading is greater than or equal to the level of the food. This is a challenging environment, requiring agents to learn to trade off between collecting food for their own and cooperating with the other agent to acquire higher team rewards. Moreover, this environment has sparse rewards making it difficult to learn and operate independently in the environment. In particular, each agent is rewarded equal to the level of the food it managed to collect, divided by its level (its contribution). Figure~\ref{fig:env-lbf} shows an illustration of this environment. 

==> chapters/08_reproducibility.tex <==
\section*{Reproducibility}
All the information for reproduction of the results can be found in Section~\ref{sec:results} with further discussions on environments in Section~\ref{appy:envs}, variations of \algo\ in Section~\ref{appy:cam_variations}, implementation details in Section~\ref{appy:implementation_details}. We also provide the code in the supplementary material with detailed explanations.
